Efficient search for superspecial hyperelliptic curves of genus four with automorphism group containing $\mathbb{Z}_6$

In arithmetic and algebraic geometry, superspecial (s.sp.\ for short) curves are one of the most important objects to be studied, with applications to cryptography and coding theory. If $g \geq 4$, it is not even known whether there exists such a curve of genus $g$ in general characteristic $p > 0$, and in the case of $g=4$, several computational approaches to search for those curves have been proposed. In the genus-$4$ hyperelliptic case, Kudo-Harashita proposed a generic algorithm to enumerate all s.sp.\ curves, and recently Ohashi-Kudo-Harashita presented an algorithm specific to the case where automorphism group contains the Klein 4-group. In this paper, we propose an algorithm with complexity $\tilde{O}(p^4)$ in theory but $\tilde{O}(p^3)$ in practice to enumerate s.sp.\ hyperelliptic curves of genus 4 with automorphism group containing the cyclic group of order $6$. By executing the algorithm over Magma, we enumerate those curves for $p$ up to $1000$. We also succeeded in finding a s.sp.\ hyperelliptic curve of genus $4$ in every $p$ with $p \equiv 2 \pmod{3}$. As a theoretical result, we classify hyperelliptic curves of genus $4$ in terms of automorphism groups in the appendix.

==> sectionA.tex <==
\appendix

\if 0
\section{Matrices of finite order and their diagonalizations}

Let $A$ be an $n \times n$ matrix over $K$.
The set $\{ p(x) \in K[x] : p(A) = O_n \}$ is an ideal of $K[x]$, and thus it is generated by a unique monic polynomial $p_A(x)$ which we call the minimal polynomial of $A$.
It is well-kwnon that $p_A(x)$ divides the characteristic polynomial $\phi_A(x) = \mathrm{det}(A - x I_n)$ of $A$, and that any eigenvalue of $A$ is a root of $p_A(x)$.
If $A$ has finite order $r$ such that $p$ does not divide $k$, then clearly $A \in \mathrm{GL}_n(K)$, and moreover $A$ is diagonalizable.
Indeed, it follows from $A^r = I_n$ that $p_A(x)$ divides $x^r - 1$.
Since $x^r-1$ has distinct roots, so is $p_A(x)$.
This means that the eigenvalues of $A$ are all different, explicitly given as $r$-th roots of unity, and also we have $n \leq r$.
Hence $A$ is diagonalizable.
Note that for any matrix $P$ composed of the eigenvectors of $A$, the diagonal matrix $P^{-1}AP$ is also of order $r$.
%Let $\lambda_1, \ldots , \lambda_n$ be the eigenvectors of $A$, and let $P=(p_1,\ldots , p_n)$ be a matrix composed of eigenvectors $p_1, \ldots , p_n$ respectively corresponding to the eigenvectors $\lambda_1, \ldots , \lambda_n$.
%It follows from $P^{-1}AP = \mathrm{diag}(\lambda_1, \ldots , \lambda_n)$ that $I_n = P^{-1}A^rP = \mathrm{diag}(\lambda_1, \ldots , \lambda_n)$ that each eigenvalue is a root $$

\begin{lemma}\label{lem:diag}
Suppose that $k$ is an algebraically closed field.
Let $A \in \mathrm{GL}_n(k)$ be a representative of an element of $\mathrm{PGL}_n(k)$.
If $A$ represents an element of $\mathrm{PGL}_n(k)$ of order $r$ such that $p$ does not divide $k$, then $A$ is diagonalizable both in $\mathrm{GL}_n(k)$ and in $\mathrm{PGL}_n(k)$.
\end{lemma}

\begin{proof}
Assume $A^r \equiv I_{n}$ in $\mathrm{PGL}_n(k)$, i.e., $A^r = a I_n$ for some $a \in k^{\times}$.
Then we have $(a^{-1/r} A)^r = a^{-1} A^r = a^{-1}(a I_n) = I_n$, and thus the eigenvalues of $a^{-1/r}A$ are all different, explicitly given as $r$-th roots of unity.
Let $\lambda_1, \ldots , \lambda_n$ be the eigenvectors of $a^{-1/r}A$, and $P$ a matrix composed of corresponding eigenvectors, say $P^{-1}(a^{-1/r}A)P = \mathrm{diag}(\lambda_1, \ldots , \lambda_n)$.
It is straightforward that $a^{1/r}\lambda_1, \ldots , a^{1/r}\lambda_n$ are the eigenvalues of $A$, and that $P^{-1} A P = a^{1/r} \mathrm{diag}(\lambda_1, \ldots , \lambda_n)$, namely $P^{-1}AP \equiv \mathrm{diag}(\lambda_1,\ldots  \lambda_r)$ in $\mathrm{PGL}_2(k)$.
\end{proof}

\begin{proof}
If one can take $a \in k$ as an element of a finite field $\mathbb{F}_q$, then clearly the order of $A$ is finite and it divides $r(q-1)$.
Since both $r$ and $q-1$ are not divided by $p$, the matrix $A$ is diagonalizable.
\end{proof}
\fi

\if 0
%===================================================
\section{Efficient isomorphism test}
%===================================================

Let $K$ be a field of characteristic $p>2$, and $\epsilon \in K^{\times} \smallsetminus (K^{\times})^2$ a non-square element.
Let $H$ be a hyperelliptic curve of genus $g$ over $K$.
Assume that $p$ and $2g+2$ are coprime.
Recall from Lemma \ref{ReductionHyper} that $H$ is given as the desingularization of the homogenization of $c y^2 = f(x)$ of the form \eqref{eq:hyp} with $c = 1$ or $\epsilon$, where $f(x)$ is a separable polynomial in $K[x]$.
Put $f(x) = \sum_{i=0}^{2g+2} a_i x^i$ with $a_i \in K$ for $0 \leq i \leq 2g+2$.
Given an $H$, we here count the number of possible equations \eqref{eq:hyp} for hyperelliptic curves isomorphic (over $K$) to $H$.

Let $H'$ be a hyperelliptic curve of genus $g$ over $K$, and $c' y^2 = \sum_{i=0}^{2g+2} a_i' x^i$ an equation for $H$ of the form \eqref{eq:hyp}.
% $\sigma : H \rightarrow H'$ an isomorphism over $K$.
By Lemma \ref{lem:isom}, a $K$-isomorphism $\sigma : H \rightarrow H'$ is given by $(x,y) \mapsto \left( \frac{\alpha x + \beta}{\gamma x + \delta}, \frac{\lambda}{(\gamma x + \delta)^{g+1}} \right)$ with
$h:=
\begin{pmatrix}
\alpha & \beta \\
\gamma & \delta
\end{pmatrix} \in \mathrm{GL}_2(K)
$ and $\lambda \in K^{\times}$, and thus $H'$ has an equation of the following form:
\begin{equation}\label{eq:H'}
c \lambda^2 y^2 =  \sum_{i=0}^{2 g + 2} a_i (\alpha x + \beta)^i (\gamma x + \delta)^{2g+2-i}.
\end{equation}
% The leading coefficient of the right hand side is $\alpha^{2 g + 2} + a_0 \gamma^{2g+2}$, which is must be nonzero.
% Putting $\mu = \alpha^{2g+2} + a_0 \gamma^{2g+2}$, we have
% \[
%  \lambda^2 \mu^{-1} y^2 =  \mu^{-1} \sum_{i=0}^{2 g + 2} a_i (\alpha x + \beta)^i (\gamma x + \delta)^{2g+2-i},
% \]
% which gives ...
This deduces a multivariate system defined by
\begin{equation}\label{eq:isom_sys}
c \lambda^2 a_{\ell}' = c' \sum_{i=0}^{2g+2} a_i \sum_{k=0}^i \binom{i}{k} \alpha^k \beta^{i-k} \binom{2g+2-i}{\ell-k} \gamma^{\ell-k} \delta^{2g+2-i- (\ell-k)} 
\end{equation}
for $0 \leq \ell \leq 2g+2$.

For the isomorphism test over $\overline{K}$, we may assume $\lambda =1$, and the cost of computing the reduced Gr\"{o}bner basis is constant in $p$.

%=============================
\subsection{Case of $\gamma = 0$}
%=============================
In this case, we have $\alpha, \delta \neq 0$ by $\mathrm{det}(h) \neq 0$, and \eqref{eq:H'} is equivalent to
\begin{equation}\label{eq:gamma_0}
c y^2 =   \left( \frac{\lambda}{\delta^{g+1}} \right)^{-2} \cdot \sum_{i=0}^{2 g + 2} a_i \left( \frac{\alpha}{\delta} x + \frac{\beta}{\delta} \right)^i =(\lambda')^{-2} \cdot \sum_{i=0}^{2 g + 2} a_i \left( \alpha' x + \beta' \right)^i ,
\end{equation}
where $\lambda' := \lambda /\delta^{g+1}$, $\alpha' := \alpha/ \delta$ and $\beta' := \beta/\delta$.
% it suffices to investigate possible values of $f_i'$.
Since
\[
(c')^{-1}a'_{2g+1} = c^{-1}(\lambda')^{-2} \left( \binom{2g+2}{1} (\alpha')^{2g+1} \beta' + a_{2g+1} \binom{2g+1}{0} (\alpha')^{2g+1} \right) ,
\]
it follows from $a_{2g+1} = a_{2g+1}' = 0$ that $c^{-1}(\lambda')^{-2} (2 g + 1) (\alpha')^{2g+1} \beta' = 0$.
By $\alpha' \neq 0$, one has $\beta' = 0$ and thus $\beta=0$. 
Hence we have
\[
(c')^{-1} a_{i}' = c^{-1} (\lambda')^{-2} a_{i} (\alpha')^{i}
\]
for each $0 \leq i \leq 2g+2$, by comparing the $x^i$-coefficient in \eqref{eq:gamma_0} with that of $c' y^2 = \sum_{i=0}^{2g+2} a'_{i} x^i$.
Considering the cases $i= 2g+2$ and $2g$, we also have $c' (\alpha')^{2g+2} = c (\lambda')^2$ and $c'(\alpha')^{2g} a_{2g} = c (\lambda')^2 a'_{2g} $, and thus $a_{2g} = (\alpha')^2 a_{2g}'$.
It follows from $c' = c (\lambda' / (\alpha')^{g+1})^{2}$ and $a_{2g} = (\alpha')^2 a_{2g}'$ that 
\begin{itemize}
\item If $c = 1$ (resp.\ $\epsilon$) then $c' = 1$ (resp.\ $\epsilon$) and $\lambda' = \pm (\alpha')^{g+1}$, and thus $a_i' = (\alpha')^{i-(2g+2)} a_i$.
\item If $a_{2g}=0$ (resp.\ $1$, $\epsilon$) then $a_{2g}' = 0$ (resp.\ $1$, $\epsilon$).
\end{itemize} 
Hence, if $a_{2g} \neq 0$, we also have $\alpha' = \pm 1$, $\lambda' = \pm 1$, and $a_i' = (\pm 1)^i a_i$ for $0 \leq i \leq 2g + 2$.
Summing up, if $\gamma = 0$, then $\alpha = \pm \delta$, $\beta = 0$ and $\lambda = \pm \delta^{g+1}$, namely,
\[
(h, \lambda) = \left(
\begin{pmatrix}
\pm \delta  & 0 \\
0 & \delta
\end{pmatrix}
, \pm \delta^{g+1} \right) \sim 
\left(
\begin{pmatrix}
\pm 1 & 0 \\
0 & 1
\end{pmatrix}
, \pm 1 \right) .
\]
The corresponding isomorphisms are $(x,y) \mapsto (x, \pm y)$ and $(x, y) \mapsto (-x, \pm y)$, and their images of $H$ are $H$ itself and $cy^2 = x^{2g+2} + \sum_{i=0}^{2g-1} (-1)^i a_{i} x^{i}$ respectively.


%================================
\subsection{Case of $\gamma \neq 0$}
%================================
In this case, the equation \eqref{eq:H'} is equivalent to
\begin{eqnarray}
c y^2 & = & \left( \frac{\lambda}{ \gamma^{g+1}} \right)^{-2} \cdot \sum_{i=0}^{2 g + 2} a_i \left( \frac{\alpha}{\gamma} x + \frac{\beta}{\gamma} \right)^i \left( x + \frac{\delta}{\gamma} \right)^{2 g + 2 - i} ,
\end{eqnarray}
namely,
\begin{eqnarray}
(\lambda')^2 c y^2 & = &  \sum_{i=0}^{2 g + 2} a_i \left( \alpha' x + \beta' \right)^i \left( x + \delta' \right)^{2 g + 2 - i}, \label{eq:gamma1}
\end{eqnarray}
where we set $\lambda' := \lambda /\gamma^{g+1}$, $\alpha' := \alpha/ \gamma$ and $\beta' := \beta/\gamma$.
The $x^{\ell}$-coefficient in the right hand side of \eqref{eq:gamma1} is
\begin{equation}\label{eq:coefficeitn}
\sum_{i=0}^{2g+2} a_i \sum_{k=\mathrm{max} \{ 0, i - (2g+2-\ell ) \}}^{\mathrm{min}\{ i, \ell \} } \binom{i}{k} (\alpha' )^k (\beta')^{i-k} \binom{2g+2-i}{\ell-k} (\delta')^{2g+2-i- (\ell-k)} .
\end{equation}
In particular, the constant term is
\begin{equation}\label{eq:const}
(\lambda')^2 c (c')^{-1} a_0' = \sum_{i=0}^{2g+2} a_i (\beta')^{i} (\delta')^{2g+2-i} ,
\end{equation}
and the $x^{2g+2}$-coefficient is
\begin{equation}\label{eq:highest}
(\lambda')^2 c (c')^{-1} = \sum_{i=0}^{2g+2} a_i (\alpha')^{i} = f(\alpha' ) \neq 0
\end{equation}
by $a_{2g+2}' = 1$.
This means that, once $\alpha'$ is determined, then $\lambda'$ and $c'$ are also determined:
If $f(\alpha')$ is a square, then $c = c' = 1$ or $c = c' = \epsilon$, and thus $\lambda' = \pm \sqrt{f(\alpha')}$.
If $f(\alpha')$ is not a square, then $c = 1$ and $c' = \epsilon$, or $c = \epsilon$ and $c' = 1$, and thus $\lambda' = \pm \sqrt{\epsilon f(\alpha')}$ or $\lambda' = \pm \sqrt{\epsilon^{-1}f(\alpha')}$.

The $x^{2g+1}$-coefficient is
\begin{eqnarray}
(\lambda')^2 c (c')^{-1} a_{2g+1}' & = & \sum_{i=0}^{2g+2} a_i \sum_{k=\mathrm{max} \{ 0, i -1 \}}^{\mathrm{min}\{ i, 2g+1 \} } \binom{i}{k} (\alpha' )^k (\beta')^{i-k} \binom{2g+2-i}{k+1-i} (\delta')^{k+1-i}  \nonumber \\
& = & a_{2g+2} (2g+2) (\alpha')^{2g+1} \beta' + a_0 (2g+2) \delta' \nonumber \\
& & + \sum_{i=1}^{2g+1} a_i \left( i (\alpha' )^{i-1} \beta' + ( 2g + 2 - i ) (\alpha' )^i \delta' \right) \nonumber \\ 
& = &  (2g+2) \beta' (\alpha')^{2g+1} + \sum_{j=0}^{2g} ( (j+1) a_{j+1} \beta' + (2g+2-j) a_j \delta' )  (\alpha')^j  \nonumber \\
& = & \left( \sum_{i=1}^{2g+2} i a_i ( \alpha' )^{i-1} \right) \beta' + \left( \sum_{i=0}^{2g+1} (2g+2-i) a_i ( \alpha' )^{i} \right) \delta' \nonumber \\
& = & f' (\alpha') \beta' + g (\alpha') \delta',\nonumber
\end{eqnarray}
and the $x^{2g}$-coefficient is
\begin{eqnarray}
& & a_{2g+2} \binom{2g+2}{2g} (\alpha')^{2g} (\beta' )^2 + a_{2g+1} \left( \binom{2g+1}{2g-1} (\alpha')^{2g-1} (\beta')^2 + \binom{2g+1}{2g} (\alpha')^{2g} (\beta') \delta' \right) \nonumber \\
& & + \sum_{i=2}^{2g} a_i \sum_{k=i-2}^i \binom{i}{k} (\alpha')^k (\beta')^{i-k} \binom{2g+2-i}{2g-k} (\delta')^{k+2-i} \nonumber \\
& & + a_1 \left( \beta' \binom{2g+1}{2g} \delta' + \alpha' \binom{2g+1}{2g-1} (\delta')^2 \right) +  a_0 \binom{2g+2}{2g} (\delta')^2 \nonumber \\
& = & \left( \sum_{i=2}^{2g+2} a_i \binom{i}{2} (\alpha')^{i-2} \right) (\beta')^2 + \left( \sum_{i=1}^{2g+1} i (2g+2-i) a_i (\alpha')^{i-1} \right) \beta' \delta'
+ \left( \sum_{i=0}^{2g} a_i \binom{2g+2-i}{2} (\alpha')^{i} \right) (\delta')^2 \nonumber \\
&=& \frac{1}{2} f'' (\alpha' ) (\beta')^2 + g' (\alpha')  \beta' \delta' - \frac{1}{2} f' (\alpha') \beta' \delta' \nonumber
\end{eqnarray}
The $x^2$-coefficient is
\begin{eqnarray}
& & a_{2g+2} \binom{2g+2}{2} (\alpha')^{2} (\beta' )^{2g} (\delta')^2 + a_{2g+1} \left( \binom{2g+1}{1} (\alpha') (\beta')^{2g} + \binom{2g+1}{2} (\alpha')^{2} (\beta')^{2g-1} \delta' \right) \nonumber \\
& & + \sum_{i=2}^{2g} a_i \sum_{k=0}^2 \binom{i}{k} (\alpha')^k (\beta')^{i-k} \binom{2g+2-i}{k} (\delta')^{2g+2-i-k} \nonumber \\
& & + a_1 \left( \beta' \binom{2g+1}{2} (\delta')^{2g-1} + \alpha' \binom{2g+1}{1} (\delta')^{2g} \right) +  a_0 \binom{2g+2}{2} (\delta')^{2g} \nonumber \\
& = & \left( \sum_{i=2}^{2g+2} a_i \binom{i}{2} (\alpha')^{i-2} \right) (\beta')^2 + \left( \sum_{i=1}^{2g+1} i (2g+2-i) a_i (\alpha')^{i-1} \right) \beta' \delta'
+ \left( \sum_{i=0}^{2g} a_i \binom{2g+2-i}{2} (\alpha')^{i} \right) (\delta')^2 \nonumber \\
&=& \frac{1}{2} f'' (\alpha' ) (\beta')^2 + g' (\alpha')  \beta' \delta' - \frac{1}{2} f' (\alpha') \beta' \delta' \nonumber
\end{eqnarray}

% and thus 
% \begin{equation}
% \beta' (\alpha')^{2g+2} + a_{2g+1} \delta' (\alpha')^{2g+1}  +  \sum_{j=0}^{2g} ( (j+1) a_{j+1} \beta' + (2g+2-j) a_j \delta' )  (\alpha')^j = 0
% \end{equation}
% by $a_{2g+1}'=0$.

Suppose $\beta' = 0$ (and thus $\beta = 0$).
In this case, it follows from $h \in \mathrm{GL}_2(K)$ that $\alpha, \alpha', \delta, \delta' \neq 0$. and \eqref{eq:coefficeitn} is
\begin{equation}
(\lambda')^2 c (c')^{-1} a_{\ell}' = \sum_{i=0}^{\ell} a_i  (\alpha' )^i  \binom{2g+2-i}{\ell-i} (\delta')^{2g+2- \ell} ,
\end{equation}
and thus
\begin{eqnarray}
0 & = &  \delta' \left( \sum_{j=0}^{2g} (2g+2-j)a_j    (\alpha')^j  \right)
\end{eqnarray}
by $a_{2g+1} = a_{2g+1}' = 0$.
Thus $\alpha'$ is a root of the polynomial of degree $2g$.
% If $a_0 \neq 0$ then $\delta' \neq 0$, and $\alpha$ is a root of the polynomial of degree $2g$.
By \eqref{eq:const}, we also have
\begin{equation}
(\lambda')^2 c (c')^{-1} a_0' = a_0 (\delta')^{2g+2} .
\end{equation}
% and
% \begin{equation}
% (\lambda')^2 c (c')^{-1} = \sum_{i=0}^{2g+2} a_i (\alpha')^{i} = f(\alpha').
% \end{equation}

Over $\overline{K}$, we may assume $c=c'=1$ and $\lambda=1$.
It follows from \eqref{eq:gamma1} that
\begin{eqnarray}
y^2 & = & \gamma^{2g+2} \sum_{i=0}^{2 g + 2} a_i \left( \alpha' x + \beta' \right)^i \left( x + \delta' \right)^{2 g + 2 - i} = f_1(x)
\end{eqnarray}
and thus 
\[
f_1(x) = \gamma^{2g+1} \sum_{i=0}^{2 g + 1} a_i \left( \alpha' x + \beta' \right)^i \left( x + \delta' \right)^{2 g + 2 - i} 
\]
by $a_{2g+2} = 0$.
Hence $f(\alpha') = f_1(-\delta') = 0$.
Considering the constant term, we also have
\[
a_{2g+1}' \sum_{i=0}^{2g+1} a_i \beta^i \delta^{2g+2-i} = a_0'(f'(\alpha) \beta + g(\alpha') \delta).
\]
Since $a_{2g+1} \neq 0$, the value of $\beta$ is determined among $2g+1$ elements if $\delta \neq 0$.
Also from the $x^{2g+1}$-coefficients, one has
\[
a_{2g+1}' = \gamma^{2g+1}(f'(\alpha) \beta + g(\alpha') \delta)
\]

%================================
\subsection{Computing automorphisms}
%================================

Automorphisms $(h, \lambda)$ with $\gamma=0$ are
\begin{itemize}
\item $(x,y) \mapsto (x, \pm y)$ and $(x, y) \mapsto (-x, \pm y)$ if $a_{2g-1} = a_{2g-3} = \cdots = a_1 = 0$.
\item Otherwise $(x,y) \mapsto (x, \pm y)$ only.
\end{itemize}

Let $(h, \lambda)$ be an automorphism of order $2$.
Then $(h^2, \lambda^2)$ is $(a I_2, a^{g+1})$ for some $a \in K \smallsetminus \{ 0 \}$.
Putting
$h:=
\begin{pmatrix}
\alpha & \beta \\
\gamma & \delta
\end{pmatrix} \in \mathrm{GL}_2(K)
$,
we have $\alpha^2 + \beta \gamma = \gamma \beta + \delta^2$, i.e., $\alpha = \pm \delta$,
$\beta (\alpha + \delta) = \gamma (\alpha + \delta) = 0$, and
$\lambda^2 = (\alpha^2 + \beta \gamma)^{g+1} = (\gamma \beta + \delta^2)^{g+1}$.


%================================
\subsection{Isomorphisms between curves in a family $H_{a,b}$}
%================================

\begin{corollary}
An isomorphism starting from $H_{a,b}$ is either of the following:
\begin{enumerate}
\item $(h, \lambda)$ with $\gamma=0$ is $(x,y) \mapsto (x, \pm y)$ only.
\end{enumerate}
\end{corollary}

The $x^9$-coefficient is
\[
0 = f' (\alpha') \beta' +  (3 a_7 (\alpha' )^7 + 6 a_4 (\alpha')^4  + 9 a_1 \alpha' ) \delta'
\]
The $x^8$-coefficient is
\begin{eqnarray}
0 & = & f''(\alpha') (\beta')^2 + (3 a_7 (\alpha' )^7 + 6 a_4 (\alpha')^4  + 9 a_1 \alpha' )' \beta' \delta' \nonumber \\
& & + (a_7 \binom{3}{2} (\alpha' )^7 + a_4 \binom{6}{2} (\alpha')^4  +  a_1 \binom{9}{2} \alpha' ) (\delta')^2. \nonumber
\end{eqnarray}
The $x^6$-coefficient is
\begin{eqnarray}
0 &=&  a_{10} \binom{10}{6} (\alpha')^6 (\beta')^4  + a_7 \sum_{k=3}^6 \binom{7}{k} (\alpha')^k (\beta')^{7-k} \binom{3}{6-k} (\delta')^{k-3} \nonumber \\
& & a_4 \sum_{k=0}^4 \binom{4}{k} (\alpha')^k (\beta')^{4-k} \binom{6}{6-k} (\delta')^{k} + a_1 \left( \beta' \binom{9}{6} (\delta')^3 + \alpha' \binom{9}{5} (\delta')^4 \right) \nonumber
\end{eqnarray}
The $x^5$-coefficient is
\begin{eqnarray}
0 &=&  a_{10} \binom{10}{5} (\alpha')^5 (\beta')^5  + a_7 \sum_{k=2}^5 \binom{7}{k} (\alpha')^k (\beta')^{7-k} \binom{3}{5-k} (\delta')^{k-2} \nonumber \\
& & a_4 \sum_{k=0}^4 \binom{4}{k} (\alpha')^k (\beta')^{4-k} \binom{6}{5-k} (\delta')^{1+k} + a_1 \left( \beta' \binom{9}{5} (\delta')^4 + \alpha' \binom{9}{4} (\delta')^5 \right) \nonumber
\end{eqnarray}
The $x^3$-coefficient is
\begin{eqnarray}
0 &=&  a_{10} \binom{10}{3} (\alpha')^3 (\beta')^7  + a_7 \sum_{k=0}^3 \binom{7}{k} (\alpha')^k (\beta')^{7-k} \binom{3}{3-k} (\delta')^{k} \nonumber \\
& & a_4 \sum_{k=0}^3 \binom{4}{k} (\alpha')^k (\beta')^{4-k} \binom{6}{3-k} (\delta')^{3+k} + a_1 \left( \beta' \binom{9}{3} (\delta')^6 + \alpha' \binom{9}{2} (\delta')^7 \right) \nonumber
\end{eqnarray}
The $x^2$-coefficient is
\begin{eqnarray}
0 &=&  a_{10} \binom{10}{2} (\alpha')^2 (\beta')^8 + a_7 \sum_{k=0}^2 \binom{7}{k} (\alpha')^k (\beta')^{7-k} \binom{3}{2-k} (\delta')^{1+k} \nonumber \\
& & a_4 \sum_{k=0}^2 \binom{4}{k} (\alpha')^k (\beta')^{4-k} \binom{6}{2-k} (\delta')^{4+k} + a_1 \left( \beta' \binom{9}{2} (\delta')^7 + \alpha' \binom{9}{1} (\delta')^8 \right) \nonumber
\end{eqnarray}
The constant term is
\begin{equation}\label{eq:Hab_const}
0 = \beta' ( (\beta')^{9} + a_7 (\beta')^6 (\delta')^3 + a_4 (\beta')^3 (\delta')^6 + a_1 (\delta')^9 )
\end{equation}
We claim $\beta' \neq 0$ and $\delta' \neq 0$.
If $\beta' = 0$, then it follows that $a_1 \alpha' \binom{9}{1} (\delta')^8 = 0$, and thus $\alpha' \delta' = 0$, which contradicts $\alpha \delta - \beta \gamma \neq 0$.
Assume $\delta' = 0$, then $(\beta')^9 = 0$ and so $\beta' = 0$, a contradiction.
If $\alpha' = 0$, then $f' (\alpha') = 0$, but $f' (0) = a_1 \neq 0$.

For each $\beta \neq 0$, it follows from \eqref{eq:Hab_const} that $\delta$ takes at most $9$ values.



\begin{enumerate}
\item For each $\beta \in \mathbb{F}_{p^2} \smallsetminus \{ 0 \}$:
\begin{enumerate}
\item Compute the roots in $\mathbb{F}_{p^2}$ of $a_1 T^9 + a_4 \beta^3 T^6 + a_7 \beta^6 T^3 + \beta^9$.
\end{enumerate}
\end{enumerate}
\fi
